Preserving Distances in Very Faulty Graphs

Preservers and additive spanners are sparse (hence cheap to store) subgraphs that preserve the distances between given pairs of nodes exactly or with some small additive error, respectively. Since real-world networks are prone to failures, it makes sense to study fault-tolerant versions of the above structures. This turns out to be a surprisingly difficult task. For every small but arbitrary set of edge or vertex failures, the preservers and spanners need to contain {\em replacement paths} around the faulted set. In this paper we make substantial progress on fault tolerant preservers and additive spanners: (1) We present the first truly sub-quadratic size single-pair preservers in unweighted (possibly directed) graphs for \emph{any} fixed number $f$ of faults. Our result indeed generalizes to the single-source case, and can be used to build new fault-tolerant additive spanners (for all pairs). (2) The size of the above single-pair preservers is $O(n^{2-g(f)})$ for some positive function $g$, and grows to $O(n^2)$ for increasing $f$. We show that this is necessary even in undirected unweighted graphs, and even if you allow for a small additive error: If you aim at size $O(n^{2-\epsilon})$ for $\epsilon>0$, then the additive error has to be $\Omega(\eps f)$. This surprisingly matches known upper bounds in the literature. (3) For weighted graphs, we provide matching upper and lower bounds for the single pair case. Namely, the size of the preserver is $\Theta(n^2)$ for $f\geq 2$ in both directed and undirected graphs, while for $f=1$ the size is $\Theta(n)$ in undirected graphs. For directed graphs, we have a superlinear upper bound and a matching lower bound. Most of our lower bounds extend to the distance oracle setting, where rather than a subgraph we ask for any compact data structure.

==> FTSPLowerbound_new.tex <==
%%\documentclass[varwidth]{standalone}
%\documentclass[a4wide]{article}
%%% HOW THIS WORKS:
%%% If you uncomment the \documentclass{article} line, then you'll be able to compile this file
%%% by itself like a normal latex file.  If you uncomment the \documentclass[varwidth]{standalone},
%%% then you can still compile this file locally, but you'll get a weird-looking pdf with no margins.
%%% But then you'll ALSO be able to compile main with this file \included.
%%% To compile locally, you'll need to include all preamble commands needed locally below.
%
%\newcommand{\eps}{\varepsilon}
%\usepackage{amsmath, amssymb, amsthm, amsfonts}
%%
%%\usepackage{graphicx}
%%
%%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{definition}[theorem]{Definition}
%
%\newcommand{\dist}{\mbox{\tt dist}}
%%
%%
%%%By Fabrizio
%%
%\usepackage{color}
%%
%
%\def\DEBUG{true}
%
%\ifdefined\DEBUG
%
%\newcommand{\mytodo}[2]{\todo[size=\tiny, color=#1!50!white]{#2}}
%
%
%\newcommand{\fab}[1]{\textcolor{red}{#1}}
% \newcommand{\mer}[1]{\textcolor{blue}{#1}}
% \newcommand{\gre}[1]{\textcolor{green}{#1}}
% \newcommand{\vir}[1]{\textcolor{cyan}{#1}}
%% \newcommand{\uri}[1]{\textcolor{magenta}{#1}}
%
%  \def\rem#1{{\marginpar{\raggedright\scriptsize #1}}}
%   \newcommand{\fabr}[1]{\rem{\textcolor{red}{$\bullet$ #1}}}
%   \newcommand{\merr}[1]{\rem{\textcolor{blue}{$\bullet$ #1}}}
%   \newcommand{\grer}[1]{\rem{\textcolor{green}{$\bullet$ #1}}}
%   \newcommand{\virr}[1]{\rem{\textcolor{cyan}{$\bullet$ #1}}}
%
%%  \newcommand{\fabr}[1]{\mytodo{red}{#1}}
%%  \newcommand{\anr}[1]{\mytodo{blue}{#1}}
%%  \newcommand{\tobr}[1]{\mytodo{green}{#1}}
%%  \newcommand{\hanr}[1]{\mytodo{cyan}{#1}}
%
%% \newcommand{\a}[1]{\mytodo{green!50!white}{#1}}
%% \newcommand{\jcom}[1]{\mytodo{red}{#1}}
%% \newcommand{\wcom}[1]{\mytodo{yellow}{#1}}
%  
%  
%  %  \newcommand{\urir}[1]{\rem{\textcolor{magenta}{$\bullet$ #1}}}
%\else
%
%  \newcommand{\fab}[1]{#1}
%  \newcommand{\an}[1]{#1}
%  \newcommand{\tob}[1]{#1}
%  \newcommand{\han}[1]{#1}
%%  \newcommand{\uri}[1]{#1}
%  \newcommand{\fabr}[1]{}
%  \newcommand{\anr}[1]{}
%  \newcommand{\tobr}[1]{}
%  \newcommand{\hanr}[1]{}
%%  \newcommand{\urir}[1]{}
%
%\fi
%
%
%\begin{document}
\vspace{-10pt}
\section{Lower Bounds for FT Preservers and Additive Spanners}
\label{sec:lbST}
In this section, we provide the first lower bound construction for a single pair $s-t$. This leads to a super-linear lower bound for FT additive spanners. We start by proving the following theorem. 
%show:\fabr{Put back a more precise claim (before missing even in appendix): more useful for future work}
  \begin{theorem}
\label{thr:LBadditive}
For any two integers $q,h>0$ and a sufficiently large $n$, there exists an unweighted undirected $n$-node graph $G = (V, E)$ and a pair $s,t\in V$ such that any $2hq$-FT $(2q-1)$-additive spanner for $G$ for the single pair $(s, t)$ has size $\Omega((\frac{n}{2hq})^{2-2/(h+1)})$.
%No $f$-FT approximate distance sensitivity oracle, even for a single $(s, t)$ demand pair, can simultaneously have strongly subquadratic space and $+o(f)$ error. 
\end{theorem}

The main building block in our lower bound is the construction of a tree $T^h$, where $h$ is a positive integer parameter related to the desired number of faults $f$. Tree $T^h$ is taken from \cite{ParterPODC15} with \fab{mild} technical adaptations. Let $d$ be a \emph{size} parameter which is used to obtain the desired number $n$ of nodes in total. 
It is convenient to interpret this tree as rooted at a specific node (though edges in this construction are undirected). We next let $rt(T^h)$ and $L(T^h)$ be the root and leaf set of $T^h$, respectively. We also let $\ell(h)$ and $n(h)$ be the height and number of nodes of $T^h$, respectively. Tree $T^h$ is constructed recursively as follows. The base case is given by $T^0$ which consists of a single isolated root node $rt(T^0)$. Note that $\ell(0)=0$ and $n(0)=1$. In order to construct $T^h$, we first create $d$ copies $T^{h-1}_0,\ldots, T^{h-1}_{d-1}$ of $T^{h-1}$. Then we add a path $v_0,\ldots,v_{d-1}$ of length $d-1$ (consisting of new nodes), and choose $rt(T^h)=v_0$. Finally, we connect $v_j$ to $rt(T^{h-1}_j)$ with a path (whose internal nodes are new) of length $(d-j)\cdot(\ell(h-1)+3)$.  This concludes the construction. See Fig. \ref{fig:lowerboundtwoST} for an illustration. Next lemma illustrates the crucial properties of $T^h$.
\begin{lemma}\label{lem:propertiesT}
The tree $T^h$ satisfies the following properties:
\begin{enumerate}\itemsep0pt
\item\label{prop:numberNodes} $n(h)\leq \frac{3}{2}(h+1)(d+1)^{h+1}$
\item\label{prop:numberLeaves} $|L(T^h)|=d^h$
\item\label{prop:faultSet} For every $\ell \in L(T^h)$, there exists $F_\ell\subseteq E(T)$,  $|F_\ell|=\fab{h}$, such that 
$\dist_{T^h\setminus F_\ell}(s, \ell) < \dist_{T^h\setminus F_\ell}(s, \ell')$ for every $\ell' \in L(T^h)\setminus \{\ell'\}$.
\end{enumerate}
\end{lemma}

\fab{***}




To prove Theorem \ref{thr:LBadditive}, we will describe the construction of a lower bound graph for FT-additive spanners. A nice feature of that graph and (most of) our other lower bound graphs constructions is that their density is due to a collection of complete bipartite graphs. Hence, using standard tools \cite{matouvsek1996distortion,bourgain1985lipschitz}\footnote{As recently applied in \cite{AmirGreg}.}, we also get strong incompressibility results for these structures; i.e. the space lower bounds apply against \emph{any} conceivable kind of approximate distance sensitivity oracle, and not just spanners. 

The main building blocks of our lower bound graph for FT-additive spanners are (1) a recursive construction of a tree $T^h$ (where $h$ is a function of the number of faults $f$), taken from \cite{ParterPODC15} with \fab{mild} technical adaptations\footnote{In \cite{ParterPODC15}, the tree $T^h$ was denoted by $G(h,d)$.}, and (2) known lower bound graphs from the theory of (non-faulty) spanners and distance preservers.

We next describe the recursive construction of the tree $T^h$ for a positive integer parameter $h$, and for a second positive integer \emph{size} parameter $d$. It is convenient to interpret this tree as rooted at a specific node (though edges in this construction are undirected). We next let $rt(T^h)$ and $L(T^h)$ be the root and leaf set of $T^h$, respectively. We also let $\ell(h)$ and $n(h)$ be the height and number of nodes of $T^h$, respectively. The base case is given by $T^0$ which consists of a single isolated root node $rt(T^0)$. Note that $\ell(0)=0$ and $n(0)=1$. In order to construct $T^h$, we first create $d$ copies $T^{h-1}_0,\ldots, T^{h-1}_{d-1}$ of $T^{h-1}$. Then we add a path $v_0,\ldots,v_{d-1}$ of length $d-1$ (consisting of new nodes), and choose $rt(T^h)=v_0$. Finally, we connect $v_j$ to $rt(T^{h-1}_j)$ with a path (whose internal nodes are new) of length $(d-j)\cdot(\ell(h-1)+3)$.  This concludes the construction. See Fig. \ref{fig:lowerboundtwoST} for an illustration. Next lemma illustrates the crucial properties of $T^h$.
\begin{lemma}\label{lem:propertiesT}
The tree $T^h$ satisfies the following properties:
\begin{enumerate}\itemsep0pt
\item\label{prop:numberNodes} $n(h)\leq \frac{3}{2}(h+1)(d+1)^{h+1}$
\item\label{prop:numberLeaves} $|L(T^h)|=d^h$
\item\label{prop:faultSet} For every $\ell \in L(T^h)$, there exists $F_\ell\subseteq E(T)$,  $|F_\ell|=\fab{h}$, such that 
$\dist_{T^h\setminus F_\ell}(s, \ell) < \dist_{T^h\setminus F_\ell}(s, \ell')$ for every $\ell' \in L(T^h)\setminus \{\ell'\}$.
\end{enumerate}
\end{lemma}


%We begin by briefly describing the lower bounds for FT preservers from \cite{ParterPODC15}. 
%The construction is based upon a tree $T^h$ rooted at the source $s$. This tree consists of a path $P$ of length $\Omega(n^{1/(h+1)})$ that originated at the source $s$, and a set of $\Omega(n^{1-1/(h+1)})$ leaf nodes $L(T^h)$. These leaf nodes are connected to the vertices on the path $P$ via a collection of paths which are defined in a recursive manner. The key property of the tree $T^h$ is the following:
%\begin{claim}
%\label{cl:helplb}
%For every leaf node $\ell \in L(T^h)$, there exists a failed set $F_\ell$ of size at most $f$, such that 
%$\dist_{T^h\setminus F_\ell}(s, \ell) < \dist_{T^h\setminus F_\ell}(s, \ell')$ for every $\ell'\neq \ell \in L(T^h)$. That is, $\ell$ is the unique closest vertex in $L(T^h)$ to $s$ in the graph $G \setminus F_\ell$.
%\end{claim}
%\vspace{-5pt}
%Let $X$ be a collection of $\Theta(n)$ vertices, and connect each of them to the last vertex of the path $P$. Finally, the lower bound graph $G$ for $f$-FT-preservers is given by adding a complete bipartite graph $B$ between $L(T^h)$ and the $X$ vertices. Thus, $G$ has $\Omega(n^{2-1/(f+1)})$ edges contributed mainly by the bipartite graph $B$. Note that indeed any edge $e=(\ell,x)$ is important for a preserver $H$, as otherwise if $e \notin H$, by Cl. \ref{cl:helplb}, $\dist_{H \setminus F_{\ell}}(s,x)>\dist_{G \setminus F_{\ell}}(s,x)$. This completes the high level description of the lower bound of \cite{ParterPODC15}. 

\paragraph{Lower bound graph for single-pair preservers and additive spanners} We now describe the graph $S^h$ that will serve as our main building block for lower bounds on $s$-$t$ preservers and spanners. We create two copies $T_s$ and $T_t$ of $T^h$. We add to $S^h$ the complete bipartite graph with sides $L(T_s)$ and $L(T_t)$, which we will call the \emph{bipartite core} of $S^h$. Observe that $|L(T_s)|=|L(T_t)|=d^h$, and hence the bipartite core contains $d^{2h}$ edges. We will call $s=sr(S^h)=rt(T_s)$ the source of $S^h$, and $t=tg(S^h)=rt(T_t)$ its target. Note that \fab{crucially the bipartite core} has $\Omega(n^{2-2/(h+1)})$ edges. We now claim that every $2h$-FT $s$-$t$ preserver $H$ for $S^{h}$ must contain each edge $e=(\ell_i,\ell_j)\in B$. Assume that $e \notin H$ and consider the case where $F_i=F_{\ell_i}$ fails in $T_{\fab{s}}$ and $F_j=F_{\ell_j}$ fails in $T_{\fab{t}}$. Recall that by Lemma \ref{lem:propertiesT}, $\ell_i$ is the closest node to $s$ in $L(T_1)$ in the graph $T_{\fab{s}}\setminus F_i$. Analogously, $\ell_j$ is the closest node to $t$ in $L(T_t)$ in the graph $T_{\fab{t}}\setminus F_j$. Hence, we conclude that $\dist_{H \setminus (F_i \cup F_j)}(s,t)>\dist_{G \setminus (F_i \cup F_j)}(s,t)$. Note that this lower bound indeed also applies to $1$-additive spanners \fab{since indeed $\dist_{H \setminus (F_i \cup F_j)}(s,t)\geq \dist_{G \setminus (F_i \cup F_j)}(s,t)+2$}. This concludes the proof of Theorem \ref{thr:LBadditive} for the case $q=1$. The same construction can also be extended to the setting of $(2h)$-FT $S\times T$ preservers. To do that, we make \emph{parallel} copies of the $S^{h}$ graphs. Details are given in Thm.\ref{thr:lowerboundST} in Appendix \ref{sec:apxLB}.  



Note that omitting one edge from the bipartite core of the graph $S^{h}$ induces a $+2$ additive stretch between $s$ and $t$ in the presence of $2h$ faults. To provide a lower bound for larger additive stretch values $2q$, we take $q$ copies $S_1,\ldots,S_q$ of the graph $S^{h}$. These copies are connected to each other by 
adding an edge between the target node of $S_i$ and the source node of $S_{i+1}$, for $i=1,\ldots,q-1$. Let $s$ be the source node of $S_1$ and $t$ be the target node of $S_q$. Overall, we get that any subgraph $H$ that has a missing edge in each one of the $q$ bipartite cores, will accumulate an additive stretch $+2q$ 
between $s$ and $t$ when a specific set of $2qh$ edges fail.\fabr{I removed "or vertices fail". We never prove anything about vertex faults here. Shall we say that this is possible?} 
This concludes the proof of Theorem \ref{thr:LBadditive} for arbitrary stretch $q$.

\fab{***}

\subsection{Lower Bound for Additive Stretch}
\begin{proof}[Proof of Thm. \ref{thr:LBadditive}]
Let us make $q$ copies $S_1,\ldots,S_q$ of graph $S^h$ with $h=f$ and $d=(\frac{n}{3q(f+1)})^{\frac{1}{f+1}}-1$. Next we chain this copies by adding one edge between $tg(S_i)$ and $sr(S_{i+1})$, for $i=1,\ldots,q-1$. We let $s=sr(S_1)$ and $t=tg(S_q)$. 

Observe that by Lemma \ref{lem:heightT-nodesT} this graph contains at most $n$ nodes, and the bipartite core of each $S_i$ has size at least $\Omega((\frac{n}{qf})^{2-2/(f+1)})$. 

Finally, we show that any $(2q-1)$-additive $s$-$t$ spanner needs to contain all the edges of at least one such bipartite core. Let us assume this does not happen, and let $e_i$ be a missing edge in the bipartite core of $S_i$ for each $i$. Observe that each $s$-$t$ shortest path has to cross $sr(S_i)$ and $tg(S_i)$ for all $i$. Therefore, it is sufficient to choose $2f$ faulty edges corresponding to each $e_i$ as in Lemma \ref{lem:sizeG}. This introduces an additive stretch of $2$ in the distance between $s$ and $t$ for each $e_i$, leading to a total additive stretch at least $2q$. 
\end{proof}

\fab{***}


%This completes the proof sketch of Theorem \ref{thr:LBadditive}. In Appendix \ref{sec:apxLB}, we prove it with many more details. 



%To build intuition, we will first describe a simpler version of the construction in which copies of $T^h$ are simply connected by complete bipartite graphs (which can be viewed as very weak distance preserver lower bound graphs).
%We will then later describe the improvements obtained by using a more interesting lower bound graph instead. 


%\paragraph{Lower bound graph for additive \fab{spanners} and one $s-t$ pair}
%Note that omitting one edge from the bipartite subgraph of the lower bound graph $S^{2f}$ induces a $+2$ additive stretch between $s$ and $t$ in the presence of $2f$ faults. To provide a lower bound for larger additive stretch values $2q$, we take $q$ copies $S_1,\ldots,S_q$ of the graph $S^{2f}$ (only that each copy contains $n/f$ vertices rather than $n$, but since the interesting $f$ values are bounded by $c\log n$, this barely affects the bounds). These copies are connected to each other by 
%adding an edge between the $t$ node of $S_i$ and the $s$ node of $S_{i+1}$, for $i=1,\ldots,q-1$. Overall, we get that any subgraph $H$ that has a missing edge in each of the $q$ bipartite subgraphs, will accumulate an additive stretch $+2q$ 
%between $s$ and $t$ when a specific set of $2q f$ edges (or vertices) fail. 
%This completes the proof sketch of Theorem \ref{thr:LBadditive}. In Appendix \ref{sec:apxLB}, we prove it with many more details. 


\paragraph{Improving over the Bipartite Core} The proof above only gives the trivial lower bound of $\Omega(n)$ for the case of two faults (using $h=\fab{q=}1$).
We can strengthen the proof in this special case to show instead that $\Omega(n^{1 + \eps})$ edges are needed:
\begin{theorem} \label{thm:subs-lb-improvement}
A $2$-FT distance preserver of a single $(s, t)$ pair needs $\Omega(n^{11/10 - o(1)})$ edges.
\end{theorem}
\vspace{-4pt}
Indeed, we
are able to show that a super-linear size is needed even in the
presence of a \emph{polynomial additive stretch}:
\begin{theorem} \label{thm:gap-pair-lb}
There are absolute constants $\eps, \delta > 0$ such that any $+n^{\delta}$-approximate $2$-FT preserver for a single $(s, t)$ pair needs $\Omega(n^{1 + \eps})$ edges in the worst case.
\end{theorem}

Finally, by tolerating one additional fault, we can obtain a strong incompressibility result:
\vspace{-4pt}
\begin{theorem} \label{thm:gap-compression-lb}
There are absolute constants $\eps, \delta > 0$ such that any $+n^{\delta}$-approximate $3$-FT distance sensitivity oracle for a single $(s, t)$ pair uses $\Omega(n^{1 + \eps})$ bits of space in the worst case.
\end{theorem}

The proofs of Theorems \ref{thm:subs-lb-improvement}, \ref{thm:gap-pair-lb} and \ref{thm:gap-compression-lb} are all given in Appendix \ref{sec:apxLB}.
The central technique in their proofs, however, is the same.
The key observation is that the structure of $T_s, T_t$ allows us to use our faults to select leaves $\ell_f, \ell_t$ and enforce that a shortest $(\ell_f, \ell_t)$ path is kept in the graph.
When we use a bipartite core between the leaves of $T_s$ and $T_t$, this ``shortest path'' is simply an edge, so the quality of our lower bound is equal to the product of the leaves in $T_s$ and $T_t$.

However, sometimes a better graph can be used instead.
In the case $h=1$, we can use a nontrivial lower bound graph against (non-faulty) subset distance preservers (from \cite{B17}), which improves the cost per leaf pair from $1$ edge to roughly $n^{11/10}$ edges, yielding Theorem \ref{thm:subs-lb-improvement}.
Alternatively, we can use a nontrivial lower bound graph against $+n^{\delta}$ spanners (from \cite{AmirGreg}), which implies Theorem \ref{thm:gap-pair-lb}.
The proof of \ref{thm:gap-compression-lb} is similar in spirit, but requires an additional trick in which \emph{unbalanced trees} are used: we take $T_s$ as a copy of $T^1$ and $T_t$ as a copy of $T^2$, and this improved number of leaf-pairs is enough to push the incompressibility argument through.


==> MultiSourceFFT-Directed_vertexfaults.tex <==
%\documentclass[11pt]{article}
%
%\usepackage[letterpaper,margin=1.00in]{geometry}
%\usepackage{amsmath, amssymb, amsthm, amsfonts}
%%\usepackage{bbm}
%
%
%%\usepackage{ifthen}
%%% \usepackage{arrayjobx}
%%\usepackage{tikz}
%%\usetikzlibrary{positioning,decorations.pathreplacing}
%
%\usepackage{cite}
%%\usepackage{url}
%\usepackage{appendix}
%\usepackage{graphicx}
%\usepackage{multirow}
%\usepackage{ragged2e}
%\usepackage{color}
%\usepackage{algorithm}
%\usepackage[noend]{algpseudocode}
%\usepackage{epstopdf}
%\usepackage{wrapfig}
%%\usepackage{paralist}
%%\usepackage{float}
%%\usepackage{pgf}
%\usepackage[textsize=tiny]{todonotes}
%\newcommand{\mtodo}[1]{\todo[color=blue!20]{#1}}
%
%% messing with tables to make them prettier
%\usepackage{array}
%\renewcommand{\arraystretch}{1.5}
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}} % horizontally centered table cells (i.e. {|P|P|P|})
%\newcolumntype{M}{>{\centering\arraybackslash}m} % also vertically centered (i.e. {|M|M|M|})
%%\newcolumntype{L}{>{\centering\arraybackslash}l} % horizontally centered table cells
%
%
%%\usepackage{framed}
%\usepackage[framemethod=tikz]{mdframed}
%%\usepackage[bottom]{footmisc}
%%\usepackage{enumitem}
%%\setitemize{noitemsep,topsep=3pt,parsep=3pt,partopsep=3pt}
%%\usepackage{multirow}
%\usepackage[font=small]{caption}
%%\captionsetup{font=small}
%\usepackage{xspace}
%\usepackage{standalone}
%
%% CL: Moved this here so it is ``seen'' by hyperref. Otherwise I got ``destination with same identifier'' issues for all theorems, lemmas, etc. with an up-to-date latex installation at home (worked on the crappy out-of-date one at work, though :D).
%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{definition}[theorem]{Definition}
%
%
%
%\definecolor{darkgreen}{rgb}{0,0.5,0}
%\usepackage{hyperref}
%\hypersetup{
%    unicode=false,          % non-Latin characters in Acrobat?‚Ç¨‚Ñ¢s bookmarks
%    colorlinks=true,        % false: boxed links; true: colored links
%    linkcolor=red,          % color of internal links (change box color with linkbordercolor)
%    citecolor=darkgreen,        % color of links to bibliography
%    filecolor=magenta,      % color of file links
%    urlcolor=cyan           % color of external links
%}
%%\usepackage[capitalize, nameinlink]{cleveref}
%%\crefformat{footnote}{#2\footnotemark[#1]#3}
%%\crefname{theorem}{Theorem}{Theorems}
%%\Crefname{lemma}{Lemma}{Lemmas}
%
%%--------------------------------------------------------------------
%\algnewcommand\algorithmicswitch{\textbf{switch}}
%\algnewcommand\algorithmiccase{\textbf{case}}
%
%% New "environments"
%\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
%\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
%\algtext*{EndSwitch}%
%\algtext*{EndCase}%
%%----------------------------------------------------------------------
%\DeclareMathOperator*{\argmin}{arg\,min}
%\newcommand{\eps}{\varepsilon}
%\newcommand{\DAS}{$\mathsf{DAS}$\xspace}
%\newcommand{\congestion}{$\mathsf{congestion}$\xspace}
%\newcommand{\dilation}{$\mathsf{dilation}$\xspace}
%\newcommand{\congest}{$\mathsf{CONGEST}$\xspace}
%\newcommand{\local}{$\mathsf{LOCAL}$\xspace}
%\newcommand{\sgn}{\operatorname{\text{{\rm sgn}}}}
%\newcommand{\poly}{\operatorname{\text{{\rm poly}}}}
%\newcommand{\floor}[1]{\lfloor #1 \rfloor}
%\newcommand{\ceil}[1]{\lceil #1 \rceil}
%\newcommand{\Fq}{\mathbb{F}_q}
%\newcommand{\prob}[1]{P(#1)}
%\newcommand{\Prob}[1]{P\left(#1\right)}
%\newcommand{\NumOfLayers}{L}
%\newcommand{\set}[1]{\left\{#1\right\}}
%\newcommand{\Hd}{\operatorname{hd}}
%\newcommand{\Wd}{\operatorname{wd}}
%\newcommand{\WD}{\operatorname{WD}}
%\newcommand{\SPD}{\operatorname{SPD}}
%\DeclareMathOperator{\E}{\mathbb{E}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\N}{\mathbb{N}}
%\def\FTBFS{\mbox{\tt FT-BFS}}
%\def\FTMBFS{\mbox{\tt FT-MBFS}}
%\def\FTMST{\mbox{\tt FT-MST}}
%\def\MST{\mbox{\tt MST}}
%\def\BFS{\mbox{\tt BFS}}
%\def\RE{\mbox{\tt SE}}
%\def\LCA{\mbox{\tt LCA}}
%\newcommand{\dist}{\mbox{\tt dist}}
%\renewcommand{\paragraph}[1]{\vspace{0.15cm}\noindent {\bf #1}:}
%\def\dnsparagraph{\paragraph}
%%--------------------------- Full Or Short --------------------------------------------- ---------------------------------------------------------------------------------------- ----------------------------------------------------------------------------------------
%
%\newcommand{\separate}[1]{\clearpage #1\clearpage} %This is for printing purposes while writing/editing
%
%\newcommand{\FullOrShort}{full}
%\def\LastE{\mbox{\tt LastE}}
%
%\ifthenelse{\equal{\FullOrShort}{full}}{
%	
%  \newcommand{\fullOnly}[1]{#1}
%  \newcommand{\shortOnly}[1]{}
%  \newcommand{\algorithmsize}{\small}
%  }{
%    %\usepackage{times}
%    % \usepackage[compact]{titlesec}
%    \renewcommand{\baselinestretch}{1.00}
%    \newcommand{\fullOnly}[1]{}
%    \newcommand{\IncludePictures}[1]{}
%   \newcommand{\algorithmsize}{\footnotesize}
%  }
%
%%-----------------------------------------------------------------------------------
%
%%By Fabrizio
%
%\usepackage{color}
%
%
%\def\DEBUG{true}
%
%\ifdefined\DEBUG
%
%\newcommand{\mytodo}[2]{\todo[size=\tiny, color=#1!50!white]{#2}}
%
%
%\newcommand{\fab}[1]{\textcolor{red}{#1}}
% \newcommand{\mer}[1]{\textcolor{blue}{#1}}
% \newcommand{\gre}[1]{\textcolor{green}{#1}}
% \newcommand{\vir}[1]{\textcolor{cyan}{#1}}
%% \newcommand{\uri}[1]{\textcolor{magenta}{#1}}
%
%  \def\rem#1{{\marginpar{\raggedright\scriptsize #1}}}
%   \newcommand{\fabr}[1]{\rem{\textcolor{red}{$\bullet$ #1}}}
%   \newcommand{\merr}[1]{\rem{\textcolor{blue}{$\bullet$ #1}}}
%   \newcommand{\grer}[1]{\rem{\textcolor{green}{$\bullet$ #1}}}
%   \newcommand{\virr}[1]{\rem{\textcolor{cyan}{$\bullet$ #1}}}
%
%%  \newcommand{\fabr}[1]{\mytodo{red}{#1}}
%%  \newcommand{\anr}[1]{\mytodo{blue}{#1}}
%%  \newcommand{\tobr}[1]{\mytodo{green}{#1}}
%%  \newcommand{\hanr}[1]{\mytodo{cyan}{#1}}
%
%% \newcommand{\a}[1]{\mytodo{green!50!white}{#1}}
%% \newcommand{\jcom}[1]{\mytodo{red}{#1}}
%% \newcommand{\wcom}[1]{\mytodo{yellow}{#1}}
%  
%  
%  %  \newcommand{\urir}[1]{\rem{\textcolor{magenta}{$\bullet$ #1}}}
%\else
%
%  \newcommand{\fab}[1]{#1}
%  \newcommand{\an}[1]{#1}
%  \newcommand{\tob}[1]{#1}
%  \newcommand{\han}[1]{#1}
%%  \newcommand{\uri}[1]{#1}
%  \newcommand{\fabr}[1]{}
%  \newcommand{\anr}[1]{}
%  \newcommand{\tobr}[1]{}
%  \newcommand{\hanr}[1]{}
%%  \newcommand{\urir}[1]{}
%
%\fi
%
%
%
%
%
%\begin{document}







%\subsection{Upper Bound}
%Let $E_f(G)=\{F \subseteq E(G) ~\mid~ |F|\leq f\}$ be the collection of all edge subsets in $G$ of size at most $f$. 
\vspace{-5pt}
\section{Efficient Construction of FT-Preservers and Spanners}
\label{sec:UB}
In this section we show:
\begin{theorem}
\label{thm:multisourcef}
For every directed or undirected unweighted graph $G=(V,E)$, integer $f \geq 1$ and $S \subseteq V$, 
one can construct in time $O(f \, n \, m)$ an $f$-FT $S$-sourcewise (i.e. $P = S \times V$) preserver of size $\widetilde{O}(f\cdot |S|^{1/2^f} \cdot n^{2-1/2^f})$. 
\end{theorem}
We remark that Theorem \ref{thm:multisourcef} holds under both edge and vertex faults. 
\fab{We next focus on the directed case, the undirected one being analogous and simpler.}\fabr{Later we talk about "directing" edges, which is not well defined for undirected graphs. So I mention that focus on directed case. In undirected case, we replace undirected edges with two directed edges, and then at the end remove directions. Shall we explain it?}

We begin by recapping the currently-known approaches for handling many vertex faults, and we explain why these approaches fail to achieve interesting space/construction time bounds for large $f$.
We then overview our new technical contributions that \fab{overcome} these barriers.
% We then explain the two challenges we are facing: the \emph{size challenge} of obtaining a structure of subquadratic size; and the \emph{time challenge} of constructing this structure in polynomial time for every number of faults $f$. 
%\vspace{-pt}
\\ 
\vspace{1pt}
\paragraph{The Size Challenge: First Attempt via Random Sampling}
\vspace{-5pt}
%\merr{This should be shorten.}
%\grer{Shortened ... check me if you'd like}
Currently, the only known approach for handling many vertex faults
%for distance preserving structures
is by \emph{random sampling} of subgraphs. This approach was introduced by Weimann and Yuster \cite{weimann2013replacement} in the setting of distance sensitivity oracles, and later on applied by Dinitz and Kraughgamer \cite{dinitz2011fault} in the setting of fault tolerant spanners. The high level idea is to generate multiple subgraphs $G_1, \ldots, G_r$ by removing each vertex with \fab{a sufficiently large} probability $p$; intuitively, each $G_i$ simultaneously captures many possible fault sets of size $f$.
%
%
% randomly over-sampling nodes to act as a fault set: Each of the $G_i$ graphs is created by removing each vertex from it with probability $p$ (to be set later). Thus, the graph $G_i$ contains $\Theta(n(1-p))$ vertices, much less than $n-f$, which allows one to capture many fault sets of size $f$ within a single graph $G_i$. 
In more detail, we say that a path $P_{s,t,F}$ is \emph{saved} in a subgraph $G_i$ if $G_i$ includes all the vertices of $P_{s,t,F}$ but none of the failed vertices of $F$ (hence, the $s-t$ shortest path in $G_i$ is precisely $P_{s,t,F}$).
Weimann and Yuster argue probabilistically that every sufficiently short replacement path of length $\le L$ is saved in some $G_i$ with high probability; thus, if we compute a (non-faulty) preserver $H_i \subseteq G_i$ for each $i$, then the graph $H = \bigcup_i H_i$ will contain every short replacement path.
For longer replacement paths that do not have this property, they decompose these paths into subpaths of length $L$ each, and use a random sampling technique to ensure that each such subpath (and thus the entire replacement path) is saved.
% that every subpath of length $L$ is saved in some $G_i$.
%They then take a random sample $B$ of $\widetilde{O}(n/L)$ vertices that ``hit'' all such subpaths with high probability.
%By also including a BFS tree rooted at $B$ in each $G_i$ in the final structure, each length $L$ subpath is thus contained in the final preserver, so the entire long replacement path is preserved.

%For each graph $G_i$, a suitable subgraph $H_i \subseteq G_i$ is computed and the final structure is the union $H=\bigcup_{i} H_i$.
%\par In more details, the random sampling approach is based upon distinguishing between \emph{short} and \emph{long} replacement paths, for a given length threshold $L$ to be defined later (i.e., a path is short if it's shorter than $L$ and otherwise, it is long)\footnote{For the setting of Dinitz and Kraughgamer \cite{dinitz2011fault}, only short replacement paths should have been saved.}.  The vertex removal probability $p$ and the number of repetitions $r$ are set such that every short replacement path $P_{u,v,F}$ is saved (there are at most $n^f$ such paths, so union bound is doable). To take care of the long replacement paths, the approach of Weimann and Yuster samples $\widetilde{O}(n/L)$ vertices $B$ that ``hit" (i.e, intersect) the long paths with high probability. 
%The resulting single source FT-preserver is given by $H=\bigcup_{i=1}^r\bigcup_{ u\in \{s\} \cup B} BFS(u,G_i).$
Unfortunately, by some straightforward algebra that we defer to the full version of this paper, we observe that any choice of parameters $p, r, L$ that ensures correctness results in $\Omega(n^2)$ or worse space usage.
We conclude that the only known approach for handling many vertex faults cannot be straightforwardly extended to produce oracles with nontrivial space usage.
%For the correctness of the construction, we need to make sure that every short replacement path is saved.
%%For simplicity, lets consider the case where $f=O(1)$.
%The probability that a short replacement path $P_{u,v,F}$ is saved by $G_i$ is 
%$q=p^{f}\cdot(1-p)^L$, and hence we must take $r=\widetilde{\Theta}(1/q)$ to guarantee that short paths are saved (w.h.p.).
%%Since the final preserver $H$ contains a BFS tree rooted at $s$ in each of the graphs $G_i$, w.h.p., it also contains the collection of all short replacement paths $P_{s,t,F}$.
%%Turning to long replacement paths $P_{s,t,F}$, here we enjoy the fact that each subpath of length $L$ intersects, w.h.p., with one of the vertices in $B$. Since all short replacement paths $P_{u,v,F}$ are saved w.h.p., and as we take into the structure all the BFS trees rooted at $B$, the correctness follows. 
%%\par We now bound the size of $H$ and show that for any setting of the parameters, the bound is $\Theta(n^2)$ and thus meaningless.
%Since our construction includes a BFS tree from the sample $B$ of $\widetilde{O}(n/L)$ BFS nodes in each $G_i$, overall the number of edges in $H$ is
%$$|E(H)|=\widetilde{O}(n^2 / L)\cdot r=\widetilde{O}(n^2 / (p^{f}\cdot(1-p)^L \cdot L)).$$
%By some straightforward algebra, which we defer to the full version of the paper, this implies that $|E(H)| = \Omega(n^2)$ for all possible parameter settings.
%First consider the case where $p\leq 1/L^{3/4}$. 
%Then, for $f\geq 2$, we get that
%$p^f (1-p)^L \cdot L \leq 1/L^{3f/4} \cdot L \leq 1/\sqrt{L}.$
%Hence, $|E(H)|\geq n^2 \cdot \sqrt{L}$. 
%Next, assume that $p> 1/L^{3/4}$, then 
%$p^f (1-p)^L \cdot L \leq (1-1/L^{3/4})^{L}\cdot L \leq e^{-L^{1/8}}.$
%Thus, again $|E(H)|\geq n^2$. 
%
In Appendix \ref{sec:apxUB}, we further discuss the size challenge and show why the common approach for $f=1$ does not extend to even $f=2$.  Thus, in the absence of new structural properties for replacement paths avoiding $f$ vertex faults, further progress, even a minor one seems very difficult.
\def\APPENDSIZECHALLENGE{
\paragraph{Second Trail: Extending the Approach of $f=1$}
%\vspace{-5pt}
We next recap the known upper bounds in the case of $f=1$, based on the ideas of \cite{roditty2012replacement,williams2011faster}. 
We then explain the barriers that have stopped prior work from easily extending this approach to $f \geq 2$.
\par This $f=1$ upper bound applies in the sourcewise setting, i.e. demand pairs $P = \{s\} \times V$.
A useful trick in analysis is to fix a target $t$ and consider its $s-t$ path $\pi(s,t)$. It is then sufficient to charge only the \emph{last} edge of each replacement path $P_{s,t,e}$ to the node $t$; the rest of the path is then charged to other nodes by an inductive argument.
%(this statement holds for any number of faults $f$).
Hence, one only needs to bound the number of \emph{new-ending} paths -- those that end in an edge that is not already in $\pi(s,t)$.
In the case $f=1$, these new-ending paths have a nice structure that has been exploited repeatedly \cite{PPFTBFS13,parter2014fault,parter2014vertex}: they diverge from $\pi(s,t)$ at some vertex $b$ above the failing vertex and collide again with $\pi(s,t)$ only at the terminal $t$\footnote{This holds so long that the shortest-paths are broken in a consistent manner.}; the subpath connecting $b$ and $t$ on the replacement path from is called the \emph{detour}.
One can divide the $s-t$ replacement paths into two groups: short (resp., long) paths are those whose detour has length at most (resp., at least) $\sqrt{n}$.
It is then straightforward enough to show that each category of path contributes only $\Oish(n^{1/2})$ edges entering $t$, and so (collecting these last edges over all nodes in the graph) the output subgraph has $\widetilde{O}(n^{3/2})$ edges in total.
%In the case of one fault, it is easy to verify that there are $\le \sqrt{n}$ edges incident to $t$ in the collection of all short paths. For the long paths, we can sample $\widetilde{O}(\sqrt{n})$ vertices $B$ which hit the detour segment of the long paths. It is then sufficient to add the $B \times \{t\}$ shortest paths computed in the graph $G^*=G \setminus (V(\pi(s,t))\setminus \{t\})$. Since by definition, the detour segment is vertex disjoint with the path $\pi(s,t)$ (except for the terminal $t$), correctness follows. In addition, we add $\widetilde{O}(\sqrt{n})$ last edges per vertex $t$, and so (collecting these last edges over all nodes in the graph) the output subgraph has $\widetilde{O}(n^{3/2})$ edges in total.
%hspace{5pt}
Generalizing this to the case of multiple faults is non-trivial already for the case of $f=2$. The main obstacle here stems from a lack of structural understanding of replacement paths for more faults: in particular, any given divergence point $b \in \pi(s,t)$ can now be associated with many new-edges and not only one!
%That is, unlike the $f=1$ setting, there might be many $P_{s,t,F}$ replacement paths that diverge from $\pi(s,t)$ at vertex $b$, each of them ending with a distinct new edge.
%When considering the long replacement paths, the situation is even less clear. In the case of one fault, we could safely omit the internal vertices on the path $\pi(s,t)$, as none of the detours used these vertices. However, once there is more then one fault, there is no one graph $G^*$ to consider, each dual failure replacement path avoids an edge which is not on $\pi(s,t)$ and hence it is not clear which subgraphs to consider in order to capture the last edges of the long replacement paths.
In the only known positive solution for $f=2$ \cite{ParterPODC15}, the approach works only for edges and is based on an extensive case analysis whose extension to larger $f$ is beyond reasonable reach.
Thus, in the absence of new structural understanding, further progress seems very difficult.
}%\APPENDSIZECHALLENGE
\\
\paragraph{The Time Bound Challenge}
%\vspace{-5pt}
A priori, it seems that constructing a preserver $H$ with $O(n^{2-\epsilon})$ edges should require computing all replacement paths $\bigcup_{s, F \subset V}P_{s,t,F}$, which leads to a construction time that scales exponentially in $f$. In particular, by deciding to omit an edge $e$ from the preserver $H$, we must somehow check that this edge does not appear on \emph{any} of the replacement paths $P_{s,t,F}$ for every $t$ and for every $F \subseteq V$, $|F|\leq f$.
Can we be sure of this without computing all the replacement paths \fab{explicitly}?
We answer this question in the affirmative and show how to compute a subquadratic-size preserver for $f=o(\log\log n)$ faults in time $O(f  n m)$.
In fact, our algorithm consists simply of $O(n)$ rounds of computation of $f$ BFS trees!
% of $n-1$ sub-routines: For each vertex $v \in V \setminus \{s\}$, it constructs $f$ BFS trees in total time of $O(f m)$. Based on these trees, it chooses which edges incident to $v$ should be added to the preserver. Hence, overall the preserver is computed by constructing $f \cdot n$ BFS trees!
The perhaps surprising correctness proof comes from the fact that each of these $f \cdot n$ BFS trees is computed in a different graph $G' \subseteq G$. Namely, for every vertex $v$ we carefully and quite nontrivially design a set of $f$ graphs that are {\em specific} to that $v$.
\\ 
\\
\paragraph{An Informal Algorithm Description}
The following description is lacking some details in order to highlight the main ideas; in particular, we omit \fab{polynomial factors in $\log n$ and $f$}.\fabr{"depend on" is too vague} We also consider the simpler case of edge faults. 
%Finally, we focus here the size of the preserver (i.e., subquadratic number of edges), rather then the time to compute it.
\hspace{5pt} We are given an unweighted graph $G=(V,E)$ and a subset of sources $S$. The goal is to construct an $f$-FT sourcewise preserver with respect to $S$.
The algorithm iterates over all nodes $t \in V$, for each it computes a subset of edges $E_t$ incident to $t$ containing the last edges of all $S \times \{t\}$ replacement paths avoiding $f$ vertex or edge faults.
The output structure $H$ is precisely the union of these $E_t$ sets.  

The computation of the \fab{sets} $E_t$ (i.e., last edges of $s-t$ replacement paths) is done in $f+1$ rounds.  Starting with $S_0=S$ and $G_0 = G$, in each round $i \in [0, f]$, we perform two tasks: (1) we add to $E_t$ the last edges that belong to the shortest paths from $S_i$ to $t$ in the graph $G_i$, and (2) we compute a new graph $G_{i+1}$ and a new node set $S_{i+1}$. We prove that any edge incident to $t$ in an {\em $(f-i)$-FT shortest path} from $S_i$ to $t$ in $G_i$ is also in an {\em $(f-i-1)$-FT shortest path} from $S_{i+1}$ to $t$ in $G_{i+1}$. The main challenge is in defining these objects.    

In our construction we have $|S_{i+1}| \gg |S_i|$ for all $i$, so the number of edges in $E_t$ is bottlenecked by the size of $S_f$, which is $|S|^{1/2^f} \cdot n^{1-1/2^f}$. Hence, the total number of edges in the structure is bounded by $n \cdot |S_f|$ (there is also an extra factor of $f$ that is necessary for technical reasons). 

The key to this argument is the reduction from an $(f-i)$-FT sourcewise preserver on $S_i$ to an $(f-i-1)$-FT sourcewise preserver on $S_{i+1}$. That is we reduce to a setting that is ``easier'' as it deals with one less fault, but we ``pay'' for it by adding more sources as $|S_{i+1}| \gg |S_i|$.  We will now overview this technique, whose key is the following inductive argument.  Assume that the bound holds for $f-1$ faults; that is, for every $n$-vertex graph, the number of edges incident to $t$ on the $S\times \{t\}$ replacement paths avoiding $\leq f-1$ faults is $O(|S|^{1/2^{f-1}}\cdot n^{1- 1/2^{f-1}})$. Now we wish to extend this claim to replacement paths that avoid $f$ faults. 
To do this, let $T_t=\bigcup_{s_i \in S}\pi(s_i,t)$ be the partial BFS tree from $S$ to $t$ (in the non-faulted graph $G$). It is more formal to view this tree as directed towards $t$, see Fig. \ref{fig:ftmulti}. Adding the edges incident to $t$ in this tree costs at most $|S|$ edges.  Hence, if $t$ has high degree in the {\em final} output structure, the density comes from the last edges of the other replacement paths $P_{s,t,F}$ for every $s \in S$,$F \subseteq E, |F|=f$.  A priori, the number of these last edges could be as large as $\Omega(n)$ and hence we might end up taking almost all edges in the graph.  We call these replacement paths whose last edge is not in $T_t$ \emph{new-ending paths}\footnote{These paths have been studied for $f\in [1,2]$ in \cite{PPFTBFS13,ParterPODC15}.}.

The crux of the analysis is to partition the new-ending paths into two classes. For each class, we will bound the number of the last edges in these paths by using the induction assumption for $f-1$ by using another set of sources $S_i \ne S$.

The first class of new-ending $S \times \{t\}$ replacement paths consists of paths whose last point $v \neq t$ at which they leave the tree $T_t$ is \emph{close} to $t$, i.e., at distance $d_i=\sqrt{n/|S|}$ or less (see the path $P_{s_1,t,F}$ in Fig. \ref{fig:ftmulti}).  The second class contains the remaining paths -- whose last point of divergence from $T_t$ is \emph{far} from $t$ (see the path $P_{s_\sigma,t,F'}$ in Fig. \ref{fig:ftmulti}). 

In each of these two classes, since we only try to bound the number of last edges, we restrict \fab{our} attention to some suffix of the replacement path and bound the number of last edges on these suffixes. 
\hspace{5pt} For the first class, we note that the detour segment starting at the last divergence point $b$ is edge disjoint with $T_t$. Hence, the detour segment from $b$ to $t$ is in fact a shortest path in $G \setminus E(T_t)\setminus F$.  We may assume that at least one of the failing edges in $F$ appears on $T_t$; else, we already have a satisfactory $b$-$t$ path.  Thus, the problem of computing last edges of the first class is reduced to a new problem in which we compute $(f-1)$-FT replacement paths between vertices $b$ and the target $t$ in the graph $G \setminus E(T_t)$. 
\par Since there are at most $\sqrt{|S|\cdot n}$ vertices at distance $\sqrt{n /|S|}$ on the tree $T_t$, we can bound the cost of these nodes by using the induction assumption for $f-1$ with $\sqrt{|S|\cdot n}$ many sources. 
\hspace{5pt} For the second class, we take a different approach.  Here, we exploit the fact the detour segment is rather long -- specifically, it has length at least $\sqrt{n/|S|}$, and hence by sampling $\widetilde{O}(\sqrt{n \cdot |S|})$ many vertices in $G$ we sample at least one node $w$ on each detour (w.h.p). Since we are only counting the last edges of these detours, it is sufficient to consider the suffix of the path starting at $w$ and ending at $t$. Again, since these detours are edge disjoint with $T_t$ and we may assume that one of the $f$ failing edges is in $T_t$, all the required last edges are contained in some $(f-1)$-FT replacement path between the hitting set and $t$ in $G \setminus E(T_t)$.  Thus, we may again reduce the problem to computing $(f-1)$-FT replacement paths from the random sample to $t$ in the graph $G \setminus E(T_t)$.  This completes our informal description.%We may again use the inductive hypothesis to bound the contribution of these paths.
%We note that idea of using hitting set for dealing with long detours has been found useful in the setting of fast computation of $1$-FT replacement paths, see e.g., \cite{roditty2012replacement,williams2011faster} and others. 

%For a preliminary high level intuition for the algorithm, see Appendix \ref{append:highlevel}.

%\begin{theorem}
%\label{thm:multisourcef}
%For every directed (or undirected) unweighted $n$-vertex graph $G=(V,E)$, integer $f \geq 1$, and $S \subseteq V$, one can construct an $f$-FT $S$-sourcewise preserver $H$ of $G$ with $\widetilde{O}(\fab{f}|S|^{1/2^f} \cdot n^{2-1/2^f})$ edges in time $O(f \cdot n \cdot m)$.
%\end{theorem}
\vspace{-1pt}
\paragraph{Algorithm for Edge Faults} Let us start with the edge faults case. The algorithm constructs a set $E_t$ of edges incident to each target node $t\in V$. The final preserver is simply the union $H= \bigcup_{t\in V} E_t$ of these edges. We next describe the construction of each $E_t$ (see also Alg. \ref{FTalgorithm}). The computation proceeds in rounds $i=0,\ldots, f$. At the beginning of round $i$ we are given a subgraph $G_i$ (with $G_0=G$) and a set of sources $S_i$ (with $S_0=S$). 

We compute a partial  
BFS tree $T_i=\bigcup_{s \in S_i} \pi_{G_i}(s,t)$\footnote{If $\pi_{G_i}(s,t)$ does not exist, recall that we define it as an empty set of edges.} from $S_i$ to $t$, and add to $E_t$ (which is initially empty) the edges $\{\LastE(\pi_{T_i}(s,t)) ~\mid~ s \in S_i\}$ of this tree incident to $t$. Here, for a path $\pi$ where one endpoint is the considered target node $t$, we denote by $\LastE(\pi)$ the edge of $\pi$ incident to $t$.
The source set $S_{i+1}$ is given by $S^{short}_i\cup S^{long}_i$. Here $S^{short}_i=\{ v \in V(T_i) ~\mid~ \dist_{T_i}(v,t) \leq d_i\}$ is the set of nodes at distance at most $d_i =\sqrt{n/|S_i|\cdot f \log n}$ from $t$, while $S^{long}_i$ is a random sample of $\Theta(n/d_i\cdot f \log n)$ vertices. 
The graph $G_{i+1}$ is obtained from $G_i$ be removing the edges $E(T_i)$\footnote{Note that for $f=1$, the algorithm has some similarity to the replacement path computation of \cite{roditty2012replacement}. Yet, there was no prior extension of this idea for $f\geq 2$.}.

\begin{algorithm}[t]
\caption{Construction of $E_t$ in our $f$-FT $S$-Sourcewise Preserver Algorithm.}
\label{FTalgorithm}
\begin{algorithmic}[1]
\Procedure{$\SWFT(t,S,f,G)$} {}
\begin{flushleft}
Input: A graph $G$ with a source set $S$ and terminal $t$, number of faults $f$. \\
Output: Edges $E_t$ incident to $t$ in an $f$-FT $S$-sourcewise preserver $H$.
\end{flushleft}
\\
Set $G_0=G$, $S_0=S$, $E_t=\emptyset$.
\For{$i \in [0,f]$}
\State Compute the partial BFS tree $T_i=\bigcup_{s \in S_i} \pi_{G_i}(s,t)$.  
\State $E_t = E_t \cup \{\LastE(\pi_{T_i}(s,t)) ~\mid~ s \in S_i\}$.
\State Set distance threshold $d_i =\sqrt{n/|S_i|\cdot f \log n}$.
\State Let $S^{short}_i=\{ v \in V(T_i) ~\mid~ \dist_{T_i}(v,t) \leq d_i\}$. 
\State Sample a collection $S^{long}_i \subseteq V(G_i)$ of $\Theta(n/d_i\cdot f \log n)$ vertices.
\State Set $S_{i+1}=S^{short}_i \cup S^{long}_i$ and $G_{i+1}=G_{i} \setminus E(T_i)$.  
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}


%The following description is lacking some details in order to highlight the main ideas; in particular, we omit factors the depend on $\log n$ and on the number of faults $f$. We also consider the more simple case of edge faults. 
%
%
%Suppose we desire an $f$-FT sourcewise preserver for a graph $G$ and source set $S$.
%Our algorithm iterates over all nodes $t \in V$ and computes a subset of edges $E_t$ incident to $t$. These subset of edges $E_t$ should contain the last edges of all $S \times \{t\}$ replacement paths avoid $f$ vertex or edge faults.
%
%The output structure $H$ is precisely the union of these sets.  The computation of $E_t$ is done in $f+1$ rounds.  Starting with $S_0=S$ and $G_0 = G$, in each round $i \in [0, f]$, we perform two tasks: (1) we add to $E_t$ the last edges that belong to the {\em non-FT} shortest paths from $S_i$ to $t$ in the graph $G_i$, and (2) we compute a new graph $G_{i+1}$ and a new node set $S_{i+1}$, and we prove that any edge incident to $t$ in an {\em $(f-i)$-FT shortest path} from $S_i$ to $t$ in $G_i$ is also in an {\em $(f-i-1)$-FT shortest path} from $S_{i+1}$ to $t$ in $G_{i+1}$. The main challenge is in defining these objects.    
%
%In our construction we have $|S_{i+1}| \gg |S_i|$ for all $i$, so the number of edges in $E_t$ is bottlenecked by the size of $S_f$, which is $|S|^{1/2^f} \cdot n^{1-1/2^f}$. Hence, the total number of edges in the structure is bounded by $n \cdot |S_f|$ (there is also an extra factor of $f$ that is necessary for technical reasons). 
%
%The key to this argument is the reduction from an $(f-i)$-FT sourcewise preserver on $S_i$ to an $(f-i-1)$-FT sourcewise preserver on $S_{i+1}$.  We will now overview this technique, whose key is the following inductive argument.  Assume that the bounds hold for $f-1$ faults; that is, for every $n$-vertex graph, the number of edges incident to $t$ on the $S\times \{t\}$ replacement paths avoiding $\leq f-1$ faults is $O(|S|^{1/2^{f-1}}\cdot n^{1- 1/2^{f-1}})$. Now we wish to extend this claim to replacement paths that avoid $f$ faults. 
%To do this, let $T_t=\bigcup_{s_i \in S}\pi(s_i,t)$ be the partial BFS tree from $S$ to $t$ (in the non-faulted graph $G$). It's convenient to view this tree as directed towards $t$. See Fig. \ref{fig:ftmulti} for an illustration. Adding the edges incident to $t$ in this tree costs at most $|S|$ edges.  Hence, if $t$ has high degree in the {\em final} output structure, the density comes from the last edges of the other replacement paths $P_{s,t,F}$ for every $s \in S$,$F \subseteq E, |F|=f$.  A priori, the number of these last edges could be as large as $\Omega(n)$ and hence we might end up taking almost all edges in the graph.  We call these replacement paths whose last edge is not in $T_t$ \emph{new-ending paths}\footnote{These paths have been studied for $f=[1,2]$ in \cite{PPFTBFS13,ParterPODC15}.}.
%
%The crux of the analysis is to partition the new-ending paths into two classes. For each class, we will bound the number of the last edges in these paths by using the induction assumption for $f-1$ by using another set of sources $S_i \ne S$.
%
%The first class of new-ending $S \times \{t\}$ replacement paths consists of paths whose last point $v \neq t$ at which they leave the tree $T_t$ is \emph{close} to $t$, i.e., at distance $d_i=\sqrt{n/|S|}$ or less (see the path $P_{s_1,t,F}$ in Fig. \ref{fig:ftmulti}).  The second class contains the remaining paths -- whose last point of divergence from $T_t$ is \emph{far} from $t$ (see the path $P_{s_\sigma,t,F'}$ in Fig. \ref{fig:ftmulti}). 
%
%In each of these two classes, since we only try to bound the number of last edges, we restrict attention to some suffix of the replacement path and bound the number of last edges on these suffixes. 
%
%For the first class, we note that the detour segment starting at the last divergence point $b$ is edge disjoint with $T_t$. Hence, the detour segment from $b$ to $t$ is in fact a shortest path in $G \setminus E(T_t)\setminus F$.  We may assume that at least one of the failing edges in $F$ appears on $T_t$; else, we already have a satisfactory $b$-$t$ path.  Thus, the problem of computing last edges of the first class is reduced to a new problem in which we compute $(f-1)$-FT replacement paths between vertices $b$ and the target $t$ in the graph $G \setminus E(T_t)$. Since there are at most $\sqrt{|S|\cdot n}$ vertices at distance $\sqrt{n /|S|}$ on the tree $T_t$, we can bound the cost of these nodes by using the induction assumption for $f-1$ with $\sqrt{|S|\cdot n}$ many sources. 
%
%For the second class, we take a different approach.  Here, we exploit the fact the detour segment is rather long -- specifically, it has length at least $\sqrt{n/|S|}$, and hence by sampling of $\widetilde{O}(\sqrt{n \cdot |S|})$ many vertices in $G$ we sample at least one node $w$ on each detour (w.h.p). Since we are only counting the last edges of these detours, it is sufficient to consider the suffix of the path starting at $w$ and ending at $t$. Again, since these detours are edge disjoint with $T_t$ and we may assume that one of the $f$ failing edges is in $T_t$, all the required last edges are contained in some $(f-1)$-FT replacement path between the hitting set and $t$ in $G \setminus E(T_t)$.  Thus, we may again reduce the problem to computing $(f-1)$-FT replacement paths from the random sample to $t$ in the graph $G \setminus E(T_t)$.  We may again use the inductive hypothesis to bound the contribution of these paths.
%
%We note that idea of using hitting set for dealing with long detours has been found useful in the setting of fast computation of $1$-FT replacement paths, see e.g., \cite{roditty2012replacement,williams2011faster} and others. 
%
%We next describe the algorithm in more details.
%
%\paragraph{Algorithm for Edge Faults}
%
%First, we will describe the algorithm for the easier case of edge faults.
%
%Fix a target $t \in V$. The algorithm computes a set of incident edges $E_t$. The output $f$-FT $S$-sourcewise preserver is then given by $H = \bigcup_{t} E_t$.  The edge set $E_t$ is computed in $f+1$ iterations. 
%Initially, set $G_0=G$, $S_0=S$,$E_t=\emptyset$. In iteration $i \in [0,f]$, we compute a (partial) BFS tree $T_i=\bigcup_{s \in S_i}\pi_{G_i}(s, t)$, and add to $E_t$ the edges incident to $t$ on $T_i$. 
%
%Then, we define a new source set $S_{i+1}$ and a new graph $G_{i+1}$ based on the tree $T_i$. Let $S_{short}^i$ be the collection of vertices on $T_i$ at distance at most $d_i=\sqrt{n/|S_i|\cdot f \log n}$ from $t$ in $G_i$ (i.e., the vertices of the first $d_i$ levels of $T_i$). Let $S_{long}^i$ be a random sample of $\Theta(n/d_i \cdot f \log n)$ vertices in $G_i$. Then, the new source set $S_{i+1}$ and new graph $G_{i+1}$ are given by $$S_{i+1}=S_{short}^i \cup 
%S_{long}^i \mbox{~~and~~} G_{i+1}=G_i \setminus E(T_i).$$ 

%
%
%\begin{mdframed}%[hidealllines=false,backgroundcolor=gray!30]
%%[hidealllines=false]
%\center \textbf{Algorithm $ComputeSourcewiseFT(t,S,f,G)$}
%\begin{flushleft}
%Input: A graph $G$ with a source set $S$ and terminal $t$, number of faults $f$. \\
%Output: Edges $E_t$ incident to $t$ in an $f$-FT $S$-sourcewise preserver $H$.
%\end{flushleft}
%\begin{itemize}
%\item Set $G_0=G$, $S_0=S$, $E_t=\emptyset$.
%\item For $i \in [0,f]$ do:
%\begin{itemize}
%\item Compute the partial BFS tree $T_i=\bigcup_{s \in S_i} \pi_{G_i}(s,t)$.  
%\item Set distance threshold $d_i =\sqrt{n/|S_i|\cdot f \log n}$.
%\item Let $S^{short}_i=\{ v \in V(T_i) ~\mid~ \dist_{T_i}(v,t) \leq d_i\}$. 
%\item Sample a collection $S^{long}_i \subseteq V(G_i)$ of $\Theta(n/d_i\cdot f \log n)$ vertices.
%\item Set $S_{i+1}=S^{short}_i \cup S^{long}_i$ and $G_{i+1}=G_{i} \setminus E(T_i)$.  
%\item $E_t = E_t \cup \{\LastE(\pi_{G_i}(s,t)) ~\mid~ s \in S_i\}$.
%\end{itemize} 
%\end{itemize}
%\end{mdframed}

%The output $f$-FT $S$-sourewise preserver $H$ is given by
%$$H= \bigcup_{t} E_t.$$

\vspace{-2pt}
\paragraph{Adaptation for Vertex Faults}
The only change in the algorithm is in the definition of the graph $G_i$ inside the procedure to compute $E_t$. We cannot allow ourselves to remove all the vertices of the tree $T_i$ from $G_i$ and hence a more subtle definition is required.
To define $G_{i+1}$, we first remove from $G_i$: (1) all edges of $S^{short}_i \times S^{short}_i$, (2)  the edges of $E(T_i)$, and (3) the vertices of $V(T_i) \setminus S^{short}_i$. In addition, we orient all remaining edges incident to $S^{short}_i$ to be directed \emph{away} from these vertices (i.e., the incoming degree of the $S^{short}_i$ vertices in $G_{i+1}$ is zero).\fabr{"direct away" was confusing since we cannot change edge directions in the directed case (not well defined for undirected)} 
In addition, we \fab{delete} all remaining edges incident to $S^{short}_i$ which are directed \fab{towards any one of} these vertices (i.e., the incoming degree of the $S^{short}_i$ vertices in $G_{i+1}$ is zero).


%In addition, we orient all remaining edges incident to $S^{short}_i$ to be directed \emph{away} from these vertices (i.e., the incoming degree of the $S^{short}_i$ vertices in $G_{i+1}$ is zero). 


\paragraph{Analysis}
We now analyze our algorithm.  Since for each vertex $t$, we compute $f$ (partial) BFS trees, we get trivially:
\vspace{-4pt}
\begin{lemma}[Running Time]\label{lem:UPtime}
The subgraph $H$ is computed within $O(f\, n\, m)$ time. 
\end{lemma}
\vspace{-4pt}
We proceed with bounding the size of $H$.
\vspace{-4pt}
\begin{lemma}[Size Analysis]\label{lem:UPsize}
$|E_t|=\widetilde{O}(|S|^{1/2^f} \cdot (fn)^{1-1/2^f})$ for every $t \in V$, hence $|E(H)|=\widetilde{O}(f|S|^{1/2^f} n^{2-1/2^f})$. 
\end{lemma}

%\def\APPENDSIZE{
\begin{proof}%[Proof of Theorem \ref{lem:UPsize}]
Since the number of edges collected at the end each round $i$ is bounded by the number of sources $S_i$, it is sufficient to bound $|S_i|$ for all $i$. Observe that, for every $i  \in [0,f-1]$, 
$$
|S_{i+1}|\leq |S^{long}_i|+|S^{short}_i| \leq d_i\cdot |S_i|+\Theta(n/d_i\cdot f \log n) =\Theta(d_i\cdot |S_i|).
$$ 
By resolving this recurrence starting with $|S_0|=|S|$ one obtains $|S_i|=O(|S|^{1/2^i}(fn\log n)^{1-1/2^i})$. The claim follows by summing over $i\in [0,f]$.
\end{proof}
%}\APPENDSIZE

%\begin{lemma}[Size Analysis]
%$|E_t|=\widetilde{O}(f^{3/2} \cdot |S|^{1/2^f} \cdot n^{1-1/2^f})$ for every $t \in V$, hence $|E(H)|=\widetilde{O}(f^{3/2} \cdot |S|^{1/2^f} \cdot n^{2-1/2^f})$. 
%\end{lemma}
%\begin{proof}
%Since the number of edges collected at the end each iteration $i$ is bounded by the number of sources $S_i$, it is sufficient to show that $S_f=\widetilde{O}(f^{1/2} n \cdot |S|^{1/2^f} \cdot n^{1-1/2^f})$. 
%To prove that, we claim that for every $i  \in [0,f-1]$, 
%\begin{equation}
%\label{eq:srec}
%|S_{i+1}|=O(d_i \cdot |S_i|)~.
%\end{equation}
%Recall that $S_{i+1}=S^{short}_i \cup S^{long}_i$ where 
%$S_{short}^i$ consists of all vertices at distance $d_i$ on the tree $T_i$. Since the tree $T_i$ has $|S_i|$ leaves, the claim holds. In addition, $|S_{long}^i|=O(f \log n \cdot n/d_i)$, which yields Eq. (\ref{eq:srec}). 
%The lemma follows by solving for $i=f$.
%\end{proof}

%\paragraph{Correctness Analysis (for vertex faults)}
We next show that the algorithm is correct. We focus on the vertex fault case, the edge fault case being similar and simpler.
Let us define, for $t\in V$ and $i \in [0,f]$,
$$
\mathcal{P}_{t,i}=\{\pi_{G_i \setminus F}(s,t) ~\mid~ s\in S_i, ~F \subseteq V(G_i),~ |F|\leq f-i\}.
$$
\vspace{-20pt}
\begin{lemma}
\label{lem:maininduc}
For every $t\in V$ and $i \in [0,f]$, it holds that:
$\LastE(\pi) \in E_t \mbox{~~for every ~~} \pi \in  \mathcal{P}_{t,i}.$
\end{lemma}
\vspace{-3pt}
\def\APPENDINDUC{
\begin{proof}[Proof of Lemma \ref{lem:maininduc}]
We prove the claim by induction on $i \in \{f, \ldots, 0\}$. For the base of the induction, consider the case of $i=f$. In this case, $\mathcal{P}_{t,f}=\{\pi_{G_f}(s,t) ~\mid~ s \in S_f\}$.  Since we add precisely the last edges of these paths to the set $E_t$, the claim holds.
Assume that the lemma holds for rounds $f, f-1, \ldots, i+1$ and consider round $i$. 
%We will prove using the induction assumption, that $\LastE(P) \in E_t$ for every $P \in \mathcal{P}_{t,i}$. 
For every $\pi_{G_i \setminus F}(s,t) \in \mathcal{P}_{t,i}$, let $P'_{s,t,F}=\pi_{G_i \setminus F}(s,t)$. \footnote{We denote these replacement paths as $P'_{s,t,F}$ as they are computed in $G_i$ and not in $G$.} 
Consider the partial BFS tree $T_i=\bigcup_{s \in S_i}\pi_{G_i}(s,t)$ rooted at $t$. 
Note that all (interesting) replacement paths $P'_{s,t,F}$ in $G_i$ have at least one failing vertex $v \in F \cap V(T_i)$ as otherwise $P'_{s,t,F}=\pi_{G_i}(s,t)$. 

We next partition the replacement paths $\pi\in\mathcal{P}_{t,i}$ into two types depending on their last edge $\LastE(\pi)$. The first class contains all paths whose last edge is in $T_i$. The second class of replacement paths contains the remaining paths, which end with an edge that is not in $T_i$. We call this second class of paths \emph{new-ending} replacement paths. Observe that the first class is taken care of, since we add all edges incident to $t$ in $T_i$. Hence it remains to prove the lemma for the set of new-ending paths. 

 
For every new-ending path $P'_{s,t,F}$, let $b_{s,t,F}$ be the last vertex on $P'_{s,t,F}$ that is in $V(T_i)\setminus \{t\}$. We call the vertex $b_{s,t,F}$ the \emph{last divergence point} of the new-ending replacement path. Note that the detour $D_{s,t,F}=P'_{s,t,F}[b_{s,t,F}\leadsto t]$ is vertex disjoint with the tree $T_i$ except for the vertices $b_{s,t,F}$ and $t$. From now on, since we only wish to collect last edges, we may restrict our attention to this detour subpath. That is, since $\LastE(D_{s,t,F})=\LastE(P'_{s,t,F})$, it is sufficient to show that $\LastE(D_{s,t,F}) \in E_t$.

Our approach is based on dividing the set of new-ending paths in $\mathcal{P}_{t,i}$ into two classes based on the position of their last divergence point $b_{s,t,F}$ (see Fig. \ref{fig:ftmulti}). The first class $\mathcal{P}_{short}$ consists of new-ending paths in $\mathcal{P}_{t,i}$ whose last divergence point is at distance at most $d_i=\sqrt{n /|S_i| \cdot f\log n}$ from $t$ on $T_i$. In other words, this class contains all new-ending paths whose last divergence point is in the set $S^{short}_i$. 
We now claim the following.
\begin{claim}
\label{cl:short}
For every $P'_{s,t,F} \in \mathcal{P}_{short}$, the detour segment $D_{s,t,F} \in \mathcal{P}_{t,i+1}$. 
\end{claim}
\begin{proof}
Since $D_{s,t,F}$ is a subpath of the replacement path $P'_{s,t,F}$, $D_{s,t,f}$ is the shortest path between $b_{s,t,F}$ and $t$ in $G_i \setminus F$. Recall that $D_{s,t,F}$ is vertex disjoint with $V(T_i) \setminus \{b_{s,t,F},t\}$. 

Since $b_{s,t,F}$ is the last divergence point of $P'_{s,t,F}$ with $T_i$, the detour $D_{s,t,F}$ starts from a vertex $b_{s,t,F} \in S^{short}_i$ and does not pass through any other vertex in $V(T_i)\setminus \{t\}$. Since we only changed in $G_{i+1}$ the direction of edges incident to $S^{short}_i$ vertices but the outgoing edge connecting $b_{s,t,F}$ to its neighbor $x$ on $D_{s,t,F}[b_{s,t,F} \leadsto t]$ remains (i.e., this vertex $x$ is not in $V(T_i) \setminus \{t\}$), this implies that the detour $D_{s,t,F}$ exists in $G_{i+1}$. In particular, note that the vertex $b_{s,t,F}$ cannot be a neighbor of $t$ in $T_i$. 
If $(b_{s,t,F},t)$ were an edge in $T_i$, then we can replace the portion of the detour path between $b_{s,t,F}$ and $t$ by this edge, getting a contradiction to the fact that $P'_{s,t,F}$ is a new-ending path\footnote{For the edge fault case, the argument is much simpler: by removing $E(T_i)$ from $G_i$, we avoid at least one the failing edges in $G_{i+1}$.}.

Next, observe that at least one of the failing vertices in $F$  occurs on the subpath $\pi_{G_i}[b_{s,t,F},t]$, let this vertex be $v \in F$. Since $v \in S^{short}_i$, all the edges are directed away from $v$ in $G_{i+1}$ and hence the paths going out from the source $b_{s,t,F}$ in $G_{i+1}$ cannot pass through $v$. Letting $F'=F \setminus V(T_i)$, it holds that (1) $|F'| \leq f-i-1$ and (2) since the shortest path ties are decided in a consistent manner and by definition of $G_{i+1}$, it holds that $D_{s,t,F}=\pi_{G_{i+1} \setminus F'}(b_{s,t,F}, t)$. As $b_{s,t,F} \in S^{short}_i$, it holds that  $D_{s,t,F} \in \mathcal{P}_{t,i+1}$.
\end{proof}
Hence by the inductive hypothesis for $i+1$, $\LastE(P'_{s,t,F})$ is in $E_t$ for every $P'_{s,t,F} \in \mathcal{P}_{short}$. 
We now turn to consider the second class of paths 
$\mathcal{P}_{long}$ which contains all remaining new-ending paths; i.e., those paths whose last divergence point is at distance at least $d_i$ from $t$ on $T_i$. Note that the detour segment $D_{s,t,F}=P'_{s,t,F}[b_{s,t,F} \leadsto t]$ of these paths is long -- i.e., length at least $d_i$. For convenience, we will consider the internal part $D'_{s,t,F}=D_{s,t,F} \setminus \{b_{s,t,F},t\}$ of these detours, so that the first and last vertices of these detour are not on $T_i$.

We exploit the lengths of these detour segments $D'_{s,t,F}$ and claim that 
 w.h.p, the set $S^{long}_i$ is a hitting set for these detours. This indeed holds by simple 
union bound overall possible $O(n^{f+2})$ detour segments. For every $P'_{s,t,F} \in \mathcal{P}_{long}$, let $w_{s,t,F} \in V(D'_{s,t,F})\cap S^{long}_i$. (By the hitting set property, w.h.p., $w_{s,t,F}$ is well defined for each long detour).
Let $W_{s,t,F}=P'_{s,t,F}[w_{s,t,F}, t]$ be the suffix of the path $P'_{s,t,F}$ starting at a vertex from the hitting set $w_{s,t,F} \in S^{long}_i$. Since $\LastE(P'_{s,t,F})=\LastE(W_{s,t,F})$, it is sufficient to show that $\LastE(W_{s,t,F})$ is in $E_t$. 
\begin{claim}
\label{cl:long} 
For every $P'_{s,t,F} \in \mathcal{P}_{long}$, it holds that the segment $W_{s,t,F} \in \mathcal{P}_{t,i+1}$. 
\end{claim}
\begin{proof}
Clearly, $W_{s,t,f}$ is the shortest path between $w_{s,t,F}$ and $t$ in $G_i \setminus F$. Since $W_{s,t,F} \subseteq D'_{s,t,F}$ is vertex disjoint with $V(T_i)$, it holds that $W_{s,t,F}=\pi_{G_{i+1} \setminus F'}(w_{s,t,F}, t)$ for $F'=F \setminus V(T_i)$. Note that since at least one fault occurred on $T_i$, we have that $|F'|\leq f-i-1$. 
As $w_{s,t,F} \in S^{long}_i$, it holds that 
$W_{s,t,F} \in \mathcal{P}_{t,i+1}$. The lemma follows.
\end{proof}
By applying the claim for $i=0$, we get that $\LastE(P'_{s,t,F})$ is in $E_t$ as required for every $P'_{s,t,F} \in \mathcal{P}_{long}$. This completes the proof.
\end{proof}
}%\APPENDINDUC
%We are now ready to complete the correctness proof.
\begin{lemma} (Correctness)\label{lem:UBcorrect}
$H$ is an $f$-FT $S$-sourcewise preserver.
\end{lemma}
\begin{proof}
By using Lemma \ref{lem:maininduc} with $i=0$, we get that for every $t \in V$, $s \in S$ and $F \subseteq V$, $|F|\leq f$, $\LastE(P_{s,t,F}) \in E_t$ (and hence also $\LastE(P_{s,t,F}) \in H$).
It remains to show that taking the last edge of each replacement path $P_{s,t,F}$ is sufficient. The base case is for paths of length $1$, where we have clearly kept the entire path in our preserver. Then, assuming the hypothesis holds for paths up to length $k-1$, consider a path $P_{s,t,F}$ of length $k$. Let $\LastE(P_{s,t,F})=(u,t)$. Then since we break ties in a consistent manner, $P_{s,t,F}=P_{s,u,F} \circ \LastE(P_{s,t,e})$. By the inductive hypothesis $P_{s,u,F}$ is in $H$, and since we included the last edge, $P_{s,t,F}$ is also in $H$. The claim follows.
\end{proof}
Theorem \ref{thm:multisourcef} now immediately follows from Lemmas \ref{lem:UPtime}, \ref{lem:UPsize}, and \ref{lem:UBcorrect}. Combing our $f$-FT sourcewise preserver from Theorem \ref{thm:multisourcef} with standard techniques (see, e.g. \cite{parter2014vertex}), in Appendix \ref{append:missproof}, we show:
\begin{theorem}
\label{thr:additivespanner}
For every undirected unweighted graph $G=(V,E)$
and integer $f\geq 1$, there exists a randomized $\Oish(fnm)$-time construction of a $+2$-additive $f$-FT spanner of $G$ of size $\widetilde{O}(f \cdot n^{2-1/(2^{f}+1)})$ \fab{that succeeds w.h.p.}\footnote{The term w.h.p. (with high probability) here indicates a probability exceeding $1-{1}/{n^c}$, for an arbitrary constant $c\geq 2$. Since randomization is only used to select hitting sets, the algorithm can be derandomized; details will be given in the journal version.}.
\end{theorem}
%Details are given in the Appendix \ref{append:missproof}. 

%\subsection{An $f$-VFT $2$-Additive Spanner} 
%
%Combing our novel $f$-FT sourcewise preserver from Theorem \ref{thm:multisourcef} with standard techniques it is easy to prove Theorem \ref{thr:addtivespanner}. 

%We next prove Theorem \ref{thr:addtivespanner}.
%This can be seen as an extension of the construction of $1$-VFT $2$-additive spanner of \cite{parter2014vertex} to the case of many vertex faults. The spanner construction works as follows. Let $L$ be an integer parameter to be fixed later. A vertex $u$ is \emph{low-degree} if it has degree less than $L$, otherwise it is \emph{high-degree}. 
%Let $S$ be a random sample of $\Theta(\frac{n}{L}\cdot f \log n)$ vertices. Our spanner $H$ consists of the $f$-VFT $S$-sourcewise preserver from Theorem \ref{thm:multisourcef} plus all the edges incident to low-degree vertices.
%
%
%%\begin{theorem}
%%\label{thr:addtivespanner}
%%There exists a (polynomially constructable) $2$-additive spanner resilient against the failing of up to $f$ (edge or vertex) faults with $\widetilde{O}(f^2 \cdot n^{2-1/(2^{f}+1)})$ edges.
%%\end{theorem}
%\begin{proof} \emph{[of Theorem \ref{thr:addtivespanner}]}
%Consider the above construction of $H$. The size of $H$ is bounded by:
%$$
%\widetilde{O}(f|S|^{1/2^f}\cdot n^{2-1/2^f})+O(n L)=\widetilde{O}(f^{1+1/2^f} L^{-1/2^f}\cdot n^{2}+ nL)
%$$
%The claim on the size follows by choosing $L=\lceil f n^{2^f/(2^f+1)}\rceil$.
%%. By Theorem \ref{thm:multisourcef}, $H_f(S)$ contains $\widetilde{O}(\fab{f}|S|^{1/2^f}\cdot n^{2-1/2^f})$ edges: by plugging the size of $|S|$, the size bound follows.
%
%Next, we turn to show correctness. First note that w.h.p every high-degree vertex has at least $f+1$ neighbors in $S$. Consider any pair of vertices $u,t$ and a set of failing vertices $F$ and let $P_{u,t,F}$ be the $u-t$ shortest path in $G\setminus F$. Let $x$ be the last vertex (closest to $t$) incident to a missing edge $e \in P_{u,t,F}\setminus E(H)$. Hence $x$ is a high-degree vertex. We observe that, w.h.p., $x$ is adjacent to at least $f+1$ vertices in $S$. Since at most $f$ vertices fail, one of the neighbors of $x$ in $S$ ,say, $s'$ survives. Let $\pi_{H\setminus F}(u, s')$ be the $u-s'$ shortest path in $H \setminus F$, and consider the following $u-t$ path $P'=\pi_{H\setminus F}(u, s')\cdot (s',x) \cdot P_{u,t,F}[x \leadsto t]$. By the definition of $x$, $P' \subseteq H$. In addition, since $H$ contains an $f$-FT $S$-sourcewise preserver and $s'\in S$, it holds that 
%\begin{eqnarray*}
%\dist_{H \setminus F}(u, t)&\leq& |P'|=\dist_{G \setminus F}(u,s')+1+|P_{u,t,F}[x \leadsto t]|
%\\&\leq&
%\dist_{G \setminus F}(u,x)+2+P_{u,t,f}[x \leadsto t]=|P_{u,t,F}|+2=\dist_{G \setminus F}(u, t) +2.
%\end{eqnarray*}
%The lemma follows.
%\end{proof}



==> PairwiseWeightedPreservers.tex <==
%\documentclass[varwidth]{standalone}
%% HOW THIS WORKS:
%% If you uncomment the \documentclass{article} line, then you'll be able to compile this file
%% by itself like a normal latex file.  If you uncomment the \documentclass[varwidth]{standalone},
%% then you can still compile this file locally, but you'll get a weird-looking pdf with no margins.
%% But then you'll ALSO be able to compile main with this file \included.
%% To compile locally, you'll need to include all preamble commands needed locally below.


%\documentclass{article}
%\usepackage{wrapfig}
%\newcommand{\eps}{\varepsilon}
%\usepackage{amsmath, amssymb, amsthm, amsfonts}
%\usepackage{graphicx}
%
%   \usepackage{color}
%
%   \newcommand{\fabr}[1]{\rem{\textcolor{red}{$\bullet$ #1}}}
%   \newcommand{\merr}[1]{\rem{\textcolor{blue}{$\bullet$ #1}}}
%   \newcommand{\grer}[1]{\rem{\textcolor{green}{$\bullet$ #1}}}
%   \newcommand{\virr}[1]{\rem{\textcolor{cyan}{$\bullet$ #1}}}
%
%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{definition}[theorem]{Definition}
%
%\newcommand{\dist}{\mbox{\tt dist}}
%
%
%\begin{document}
\vspace{-5pt}
\section{FT Pairwise Preservers for Weighted Graphs}
\label{sec:Weighted}
We now turn to consider weighted graphs, for which the space requirements for $s-t$ FT preservers are considerably larger. In Appendix \ref{sec:apxWeighted}, we show:
\begin{theorem} \label{thm:uwstub}
For any undirected weighted graph $G$ and pair of nodes $(s, t)$, there is a $1$-FT $s$-$t$ preserver with $O(n)$ edges.
\end{theorem}
With a trivial union bound, we get that any set $P$ of node pairs can be preserved using $O(\min(n|P|, n^2))$ edges.  It is natural to wonder if one can improve this union bound by doing something slightly smarter in the construction.
Surprisingly, the answer is no: we are able to provide a matching lower bound for Theorem \ref{thm:uwstub}.
%\begin{theorem}\label{thr:UBqpairs}
%For any $q \le n$, there exists an undirected weighted graph $G$ and a set $Q$ of $q$ node pairs such that every $1$-FT preserver of $G, Q$ has $\Omega(n|Q|)$ edges.
%\end{theorem}
\begin{theorem} 
\label{thr:UBqpairs}
For any integer $1\leq p \leq {n\choose 2}$, there exists an undirected weighted graph $G$ and a set $P$ of $p$ node pairs such that every $1$-FT $P$-pairwise preserver of $G$ contains $\Omega(\min(np, n^2))$ edges.
\end{theorem}
\begin{proof}
%This proof is an adaptation of Lemma \ref{lem:sizeG}.%\cite{PPFTBFS13}.
We construct our lower bound instance by adapting the construction in Lemma \ref{lem:sizeG}.  First, add a path of length $n+1$ using edges of weight $1$.  Call the nodes on the path $p_1, \dots, p_{n+1}$.  Next, create $n$ new nodes $\{v_i\}$, and add an edge of weight $1$ from $p_{n+1}$ to each $v_i$.  Then, for each $i \in [1, p]$, add a new node $x_i$ to the graph, and connect $x_i$ to $p_i$ with an edge of weight $2(n - i) + 1$.  Finally, for all $i \in [1, p], j \in [1, n]$, add an edge of weight $1$ between $x_i$ and $v_j$.

Define the pair set $P$ to be $\{s\} \times \{v_i \ \mid \ i \in [1, p]\}$.  Note that the graph has $\Theta(n)$ nodes and $\Omega(n|P|)$ edges, because there are exactly $n|P|$ edges between the nodes $\{x_i\}$ and $\{v_j\}$.  We will complete the proof by arguing that all edges in $\{x_i\} \times \{v_j\}$ must be kept in the preserver.  Specifically, we claim that for any $i, j$, the edge $(x_i, v_j)$ is needed to preserve the distance of the pair $(s, v_j) \in P$ when the edge $(p_i, p_{i+1})$ faults.  To see this, note that any path from $s$ to $v_j$ must pass through {\em some} node $x_i$, and we have $\dist(s, x_i) = (i-1) + 2(n-i) + 1 = 2n - i$ for any $i$.  Since $(p_i, p_{i+1})$ has faulted, the path from $s$ to $v_j$ must intersect $x_{i'}$ for some $i' \le i$ before it intersects $x_{i''}$ for any $i'' > i$.  Therefore, the shortest $s-v_j$ path passes through $x_i$, and thus uses $(x_i, v_j)$.
\end{proof}
Many remaining results for weighted FT preservers are in Appendix \ref{sec:apxWeighted}.

%\end{document}

==> UpperBoundAdditive.tex <==
%\documentclass[varwidth]{standalone}
%\documentclass{article}
%% HOW THIS WORKS:
%% If you uncomment the \documentclass{article} line, then you'll be able to compile this file
%% by itself like a normal latex file.  If you uncomment the \documentclass[varwidth]{standalone},
%% then you can still compile this file locally, but you'll get a weird-looking pdf with no margins.
%% But then you'll ALSO be able to compile main with this file \included.
%% To compile locally, you'll need to include all preamble commands needed locally below.

%\usepackage{amsthm, amsmath}
%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{definition}[theorem]{Definition}
%
%\newcommand{\eps}{\varepsilon}
%
%\usepackage[letterpaper,margin=1.00in]{geometry}
%
%
%\begin{document}

\subsection{Upper Bounds for FT-Additive Spanners}

\paragraph{Additive Stretch 2}
\begin{lemma}
\label{lem:addtivespanner}
There exists a (polynomially constructable) $2$-additive spanner resilient against the failing of up to $f$ (edge or vertex) faults with $\widetilde{O}(f^2 \cdot n^{2-1/(2^{f}+1)})$ edges.
\end{lemma}
\begin{proof}
A vertex $u$ is \emph{low-degree} if it has less than $\Theta(f \cdot n^{2^f/(2^f+1)}\cdot \log n)$ edges, otherwise it is high-degree. 
Let $S$ be a random sample of $\Theta(f \log n \cdot n^{1/(2^f+1)})$ vertices in $V$. 
The spanner $H$ consists of the $f$-FT $S \times V$ preserver $H_f(S)$ and the edges incident to all low-degree vertices.

We first bound the size of $H$. By Lemma \ref{thm:multisourcef}, $H_f(S)$ contains $\widetilde{O}(f^{3/2}|S|^{1/2^f}\cdot n^{2-1/2^f})$ edges by plugging the size of $|S|$, the size bound follows.

Next, we turn to show correctness. Consider any pair of vertices $u,t$ and a set of failing edges $F$ and let $P_{u,t,F}$ be the $u-t$ shortest path in $G$. Let $x$ be the last vertex (closest to $t$) incident to a missing edge in $e \in P_{s,t,F}\setminus E(H)$. Hence $x$ is a high-degree vertex. In particular, w.h.p., $x$ is adjacent to $f+1$ vertices in $S$. Since at most $f$ edges fails, one of the edges $e'$ connecting it to a vertex, say, $s'$ in $S$ survives. Let $\pi_{H\setminus F}(u, s')$ be the $u-s'$ shortest path in $H \setminus F$, and consider the following $u-t$ path $P'=\pi_{H\setminus F}(u, s')\cdot e' \cdot P_{u,t,f}[x \leadsto t]$. By the definition of $x$, $P' \subseteq H$. In addition, since $H$ constains an $f$-FT-BFS with respect to $s'$, it holds that 
\begin{eqnarray*}
\dist_{H \setminus F}(u, t)&\leq& |P'|=\dist_{G \setminus F}(u,s')+1+|P_{u,t,f}[x \leadsto t]|
\\&\leq&
\dist_{G \setminus F}(u,x)+2+P_{u,t,f}[x \leadsto t]=|P_{u,t,f}|+2=\dist_{G \setminus F}(u, t)~.
\end{eqnarray*}
The lemma follows.
\end{proof}
%
%\paragraph{Additive Stretch 4}
%\begin{lemma}
%\label{lem:addtivespanner}
%There exists a (polynomial-time constructible) $4$-additive spanner resilient against the failing of up to $f$ (edge or vertex) faults with $\widetilde{O}(n^{2-1/(2^{f-1}+1)})$ edges.
%\end{lemma}
%\begin{proof}
%TBA
%\end{proof}
%\paragraph{$D$-preservers}\fabr{I would skip this par. Not very interesting and we have enough results. \mer{I know that people care about $D$-preservers, they got attention in Virgi, Amir and Greg's papers. But, I do not mind removing it.}}
%We now claim that the structure $H_f(S)$ can also yield fault tolerant subgraphs for $D$ threshold preservers. 
%\cite{celkin} introduced the
%$D$-preservers structures -- subgraphs that  preserve
%the distances between all pairs of vertices that are at
%distance at least $D$. \cite{celkin}  showed a matching result of $O(n^2/D)$ bound for these objects. The fault tolerant version of $D$-preservers denote by $f$-FT-$D$-\emph{preservers} are subgraphs $H_f(D) \subseteq G$ satisfying $\dist_{H_f(D) \setminus F}(s,t)=\dist(s,t, G \setminus F)$ for every $s-t$ of distance at least $D$ in $G$ and for every $F \subseteq E$, $|F|\leq f$. 

%
%\end{document}
